Model-Based Monitoring for IoTs Smart Cities Applications

Smart Cities are future urban aggregations, where a multitude of heterogeneous systems and IoT devices interact to provide a safer, more efficient, and greener environment. The vision of smart cities is adapting accordingly to the evolution of software and IoT based services. The current trend is not to have a big comprehensive system, but a plethora of small, well integrated systems that interact one with each other. Monitoring these kinds of systems is challenging for a number of reasons.

==> ack.tex <==
\begin{small}
\section*{Acknowledgment}
This work has been partially supported by the H2020 Learn project, which has been funded under the ERC Consolidator Grant 2014 program (ERC Grant Agreement n. 646867); by the Italian Ministry of Education, University, and Research (MIUR) with the PRIN project GAUSS (grant n.~2015KWREMX), and by the H2020 NGPaaS project (grant n.~761557).
\end{small}	
